Video World Models with Long-term Spatial Memory

Emerging world models autoregressively generate video frames in response to actions, such as camera movements and text prompts, among other control signals. Due to limited temporal context window sizes, these models often struggle to maintain scene consistency during revisits, leading to severe forgetting of previously generated environments. Inspired by the mechanisms of human memory, we introduce a novel framework to enhancing long-term consistency of video world models through a geometry-grounded long-term spatial memory. Our framework includes mechanisms to store and retrieve information from the long-term spatial memory and we curate custom datasets to train and evaluate world models with explicitly stored 3D memory mechanisms. Our evaluations show improved quality, consistency, and context length compared to relevant baselines, paving the way towards long-term consistent world generation.

==> tables/taxonomy.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{\textbf{Comparison with different spatial-aware video generative models}}
    \small
    \begin{tabular}{l|l|cccc}
    \toprule
    \multicolumn{2}{l|}{Methods} & Cam-Ctrl & Long-Mem & Action-Pred & S/D-Decouple \\
    \midrule
    Point condition & \cite{yu2024viewcrafter,gu2025das,yu2025trajectorycrafter,ren2025gen3c} & \ding{51} & \ding{55} & \ding{55} & \ding{55} \\
    \multirow{2}[0]{*}{Camera condition} & \cite{wang2024motionctrl,bahmani2025vd3d,bahmani2025ac3d,he2025cameractrl2} & \ding{51} & \ding{55} & \ding{51} & \ding{55} \\
          & \cite{zhang2024recapture,bai2025syncammaster,bai2025recammaster} & \ding{51} & \ding{55} & \ding{55} & \ding{55} \\
    Hidden state & \misscite{Po's}  & \ding{51} & \ding{51} & \ding{51} & \ding{55} \\
    History frames & \cite{xiao2025worldmem} & \ding{51} & \ding{51} & \ding{51} & \ding{55}  \\
    \midrule
    \multicolumn{2}{l|}{\textbf{Ours}} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
    \bottomrule
    \end{tabular}%
  \label{tab:taxonomy}%
\end{table}%

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[t]
%   \centering
%   \caption{\textbf{Comparison with different spatial-aware video generative models}}
%     \small
%     \begin{tabular}{l|l|ccccc}
%     \toprule
%     \multicolumn{2}{l|}{Methods} & Cam-Ctrl & Long-Mem & Action-Pred & S/D-Decouple & Domain \\
%     \midrule
%     Point condition & \cite{yu2024viewcrafter,gu2025das,yu2025trajectorycrafter,ren2025gen3c} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & Real-world \\
%     \multirow{2}[0]{*}{Camera condition} & \cite{wang2024motionctrl,bahmani2025vd3d,bahmani2025ac3d,he2025cameractrl2} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & Real-world \\
%           & \cite{zhang2024recapture,bai2025syncammaster,bai2025recammaster} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & Real-world \\
%     Hidden state & \misscite{Po's}  & \ding{51} & \ding{51} & \ding{51} & \ding{55} & MineCraft \\
%     History frames & \cite{xiao2025worldmem} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & MineCraft/Static scenes \\
%     \midrule
%     \multicolumn{2}{l|}{\textbf{Ours}} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & Real world \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:taxonomy}%
% \end{table}%

